Adaptive Bayesian density estimation using Pitman-Yor or normalized inverse-Gaussian process kernel mixtures

We consider Bayesian nonparametric density estimation using a Pitman-Yor or a normalized inverse-Gaussian process kernel mixture as the prior distribution for a density. The procedure is studied from a frequentist perspective. Using the stick-breaking representation of the Pitman-Yor process or the expression of the finite-dimensional distributions for the normalized-inverse Gaussian process, we prove that, when the data are replicates from an infinitely smooth density, the posterior distribution concentrates on any shrinking $L^p$-norm ball, $1\leq p\leq\infty$, around the sampling density at a \emph{nearly parametric} rate, up to a logarithmic factor. The resulting hierarchical Bayesian procedure, with a fixed prior, is thus shown to be adaptive to the infinite degree of smoothness of the sampling density.

==> table1.tex <==
% matrix: b file: table1.tex  14 Sep 2001 18:06:44
\begin{table}[htbp]
%\caption{Estimated Parameters}
\label{table:one}
\begin{center}
%\caption{Estimated Parameters}\centering\medskip
\begin{tabular}{|l|l|l|}\hline
 & weight  & cons  \\ \hline
y1 & -.00600869 & 39.440284 \\ \hline
\end{tabular}
\caption{Estimated Parameters}
\end{center}
\end{table}

